Hierarchical Decoupling Capacitor Optimization for Power Distribution Network of 2.5D ICs with Co-Analysis of Frequency and Time Domains Based on Deep Reinforcement Learning

With the growing need for higher memory bandwidth and computation density, 2.5D design, which involves integrating multiple chiplets onto an interposer, emerges as a promising solution. However, this integration introduces significant challenges due to increasing data rates and a large number of I/Os, necessitating advanced optimization of the power distribution networks (PDNs) both on-chip and on-interposer to mitigate the small signal noise and simultaneous switching noise (SSN). Traditional PDN optimization strategies in 2.5D systems primarily focus on reducing impedance by integrating decoupling capacitors (decaps) to lessen small signal noises. Unfortunately, relying solely on frequency-domain analysis has been proven inadequate for addressing coupled SSN, as indicated by our experimental results. In this work, we introduce a novel two-phase optimization flow using deep reinforcement learning to tackle both the on-chip small signal noise and SSN. Initially, we optimize the impedance in the frequency domain to maintain the small signal noise within acceptable limits while avoiding over-design. Subsequently, in the time domain, we refine the PDN to minimize the voltage violation integral (VVI), a more accurate measure of SSN severity. To the best of our knowledge, this is the first dual-domain optimization strategy that simultaneously addresses both the small signal noise and SSN propagation through strategic decap placement in on-chip and on-interposer PDNs, offering a significant step forward in the design of robust PDNs for 2.5D integrated systems.

==> tex/3related.tex <==
\section{Related Work}
\label{related work}

In the field of circuits and systems, various methods of decap design optimization have been proposed based on the conventional optimization algorithms, such as the genetic algorithm (GA) \cite{piersanti2017decoupling,de2020genetic,xu2021jitter}, particle swarm optimization (PSO) algorithm \cite{kadlec2018pcb,hemaram2021optimal} and simulated annealing (SA) algorithm \cite{zhao2002decoupling,tripathi2017minimizing,chen2023interposer}. GA-based methods can explore a large search space efficiently, but they may struggle to capture sequential combinational relationships between decap assignments and other meta-features, such as the position of probing ports. PSO algorithms, on the other hand, offer fast convergence speeds and simple coding structures. However, they are prone to fall into the local optima, which prevents them from reaching the global optimum solution. Although SA algorithms possess the ability to escape local optima due to their probabilistic acceptance of worse solutions, they have lower convergence rates compared to PSO algorithms and require a good initial solution to perform effectively. None of these optimization algorithms can guarantee finding the optimal solution, especially when dealing with a large number of decap locations. Besides, the optimization time can become problematic, particularly when considering a vast search space. The fusion of differential evolution (DE), which has a strong global search ability, with PSO algorithms enables the optimization of decap designs for 2.5D systems \cite{zhi2022trade}. However, this approach specifically focuses solely on optimizing the on-interposer decap, assuming that chiplets are fully designed and plug-and-play. 

RL has indeed gained traction in addressing complex tasks, especially decap optimization.  Several methods utilizing RL for decap optimization have been proposed in the literature \cite{park2018reinforcement,park2020deep,park2022transformer,zhang2023decoupling}. Value-based RL methods using the Q-learning algorithm have been explored for decap placement optimization \cite{park2018reinforcement,park2020deep}. However, they consider a single probing port and encounter limitations regarding solution space size and high computing costs. To increase the space size and generalization ability, a transformer network-based method for PDN decap optimization of high bandwidth memory (HBM) was proposed \cite{park2022transformer}. The method can optimize decap design to maximize the reduction of both the self- and transfer impedances seen at multiple ports. Additionally, another RL-based approach \cite{zhang2023decoupling} optimizes the locations of decaps with different capacitance, considering the complex PDN structure with irregular shapes typical of printed circuit boards (PCBs). This method demonstrates greater scalability compared to the approaches \cite{park2018reinforcement,park2020deep,park2022transformer} that support only one decap capacitance.

Most of the previous decap optimization methods have primarily focused on maximizing the reduction of impedance in the frequency domain \cite{piersanti2017decoupling,de2020genetic,xu2021jitter,kadlec2018pcb,hemaram2021optimal,zhao2002decoupling,tripathi2017minimizing,chen2023interposer,zhi2022trade,park2018reinforcement,park2020deep,park2022transformer,zhang2023decoupling}. However, relying solely on frequency-domain analysis cannot capture the impact of transient responses on the circuit, making it challenging to predict whether the voltage noise meets design requirements. Su \textit{et al.} \cite{su2003optimal} and Enami \textit{et al.} \cite{enami2008decoupling} have investigated the time-domain %\st{evaluation methods for the} 
decap optimization \LLS{methods for on-chip PDNs only, which are not designated for 2.5D systems}. %\LLS{Moreover, pure time-domain methods could be time-consuming without impedance characteristics across different frequencies.}


